Stability and Instability of the MaxWeight Policy

Consider a switched queueing network with general routing among its queues. The MaxWeight policy assigns available service by maximizing the objective function $\sum_j Q_j \sigma_j$ among the different feasible service options, where $Q_j$ denotes queue size and $\sigma_j$ denotes the amount of service to be executed at queue $j$. MaxWeight is a greedy policy that does not depend on knowledge of arrival rates and is straightforward to implement. These properties, as well as its simple formulation, suggest MaxWeight as a serious candidate for implementation in the setting of switched queueing networks; MaxWeight has been extensively studied in the context of communication networks. However, a fluid model variant of MaxWeight was shown by Andrews--Zhang (2003) not to be maximally stable. Here, we prove that MaxWeight itself is not in general maximally stable. We also prove MaxWeight is maximally stable in a much more restrictive setting, and that a weighted version of MaxWeight, where the weighting depends on the traffic intensity, is always stable.

==> 5-BRANCHING_MERGING.tex <==
% !TeX root    = MOR-PAPER.tex
\section{Priority through Branching and Merging} \label{sec:BranchMerge}


\color{magenta}
On positive results for single class:

--  General case is done in Ã¢ÂÂtoneil5.1.16Ã¢ÂÂ.  Although it refers back to the more concrete cases (e.g., toneil3.16.16), it seems that the reasoning is complete.

--  Ã¢ÂÂtomaury5.6.16Ã¢ÂÂ is from Bernardo, with modifications of my 5.1.16 version in blue.  Looking at it quickly, it seems that Bernardo essentially fills in a few steps from the 5.1.16 message and introduces the (accidentally) suppressed argument t in a few places.  I donÃ¢ÂÂt agree with all of the changes (which I have just quickly scanned), for instance, re-using c(t) for the Ã¢ÂÂobjective functionÃ¢ÂÂ  (when $c_k$ is already used) and using the mixed vector-coordinate notation there.  Also note that my referring to f(t) a few lines lower down as the Lyapunov function is misleading, since it is h(t), rather than f(t), which is decreasing.  

On correspondence not in the Dropbox folder:

--  A good chunk of this is in the email thread titled:  MaxWeight single class , which extends from 2/2/16 to 7/7/16.  At some point, we should look all of this over to make sure something isnÃ¢ÂÂt being forgotten (although a lot is presumably outmoded).  

-------  This includes some (preliminary) suggestions by me on 5/3/16 on the organization of the paper (which has presumably been superseded).  

-------  This also includes my response on 5/6/16 to BernardoÃ¢ÂÂs corrections on the same date -- I see that this includes my comments above.  

-------  In the next few messages, there is a discussion between Neil and me on the roles of branching and funneling (aka merging) in creating instability.  At this point, this is vague in my mind, but I remember the issue of the Ã¢ÂÂcorrectÃ¢ÂÂ philosophical point of view of Ã¢ÂÂwhat causes the instabilityÃ¢ÂÂ as being unresolved.  Neil forced me to backtrack from some of my initial ideas.

--  This discussion of branching/funneling (aka, merging) continues in the email thread titled:  Maxweight (continued) that is dated 7/20/16.  

--  Another email thread to look at is:  Instability Paper Version 1, dated 10/3/16.  I havenÃ¢ÂÂt gone through this carefully, but I see that on 9/25/16, I had some criticisms of NeilÃ¢ÂÂs initial write-up; I expressed more of these in phone conversations.   I had some serious reservations about the material there (how it was written/presented, and the role it should play in the eventual paper), it didnÃ¢ÂÂt want to consider its inclusion as a done deal.  This is what I was referring to in last FridayÃ¢ÂÂs Skype conversation.  

--  There were additional sketches by me on how to construct various counterexamples in the multiclass case, as well as correspondence with Neil on his way of getting a positive result in that framework.  These are both outlined in my UCSD talk, which you both have.  I havenÃ¢ÂÂt located this, but presumably could with more effort.  (If you wish to see this, let me know.) 

This outline hopefully helps, but it certainly will not contain everything.  For instance, Neil pointed out that one can use our purely MaxWeight Lyapunov function (instead of its generalization) when there is parallel routing, even if the rates are not identical.  

A general request for future email correspondence;  the lines in some of the past messages have exceeded the width of my computer screen, so IÃ¢ÂÂve had to do a lot of back and forth to read individual lines.  So, please try to keep the lines within standard length.  (If you know a way I can solve this problem, IÃ¢ÂÂd of course like to hear it.)
\color{black}  
